Exclusive J/$\psi$ Detection and Physics with ECCE

Exclusive heavy quarkonium photoproduction is one of the most popular processes in EIC, which has a large cross section and a simple final state. Due to the gluonic nature of the exchange Pomeron, this process can be related to the gluon distributions in the nucleus. The momentum transfer dependence of this process is sensitive to the interaction sites, which provides a powerful tool to probe the spatial distribution of gluons in the nucleus. Recently the problem of the origin of hadron mass has received lots of attention in determining the anomaly contribution $M_{a}$. The trace anomaly is sensitive to the gluon condensate, and exclusive production of quarkonia such as J/$\psi$ and $\Upsilon$ can serve as a sensitive probe to constrain it. In this paper, we present the performance of the ECCE detector for exclusive J/$\psi$ detection and the capability of this process to investigate the above physics opportunities with ECCE.

==> institute_list.tex <==
\newcommand\AANL[1] {\ifnum#1=1 1\else\fi}
\newcommand\AcademiaSinica[1] {\ifnum#1=1 2\else Institute of Physics, Academia Sinica, Taipei, Taiwan\fi}
\newcommand\AUGIE[1] {\ifnum#1=1 3\else Augustana University, Sioux Falls, SD, USA\fi}
\newcommand\BGU[1] {\ifnum#1=1 4\else\fi}
\newcommand\BNL[1] {\ifnum#1=1 5\else Brookhaven National Laboratory, Upton, NY, USA\fi}
\newcommand\BrunelUniversity[1] {\ifnum#1=1 6\else Brunel University London, Uxbridge, UK\fi}
\newcommand\CanisiusCollege[1] {\ifnum#1=1 7\else Canisius College, Buffalo, NY, USA\fi}
\newcommand\CCNU[1] {\ifnum#1=1 8\else Central China Normal University, Wuhan, China\fi}
\newcommand\Charles[1] {\ifnum#1=1 9\else Charles University, Faculty of Maths and Physics, Prague, Czech Republic\fi}
\newcommand\CIAE[1] {\ifnum#1=1 10\else China Institute of Atomic Energy, Fangshan, Beijing, China\fi}
\newcommand\CNU[1] {\ifnum#1=1 11\else Christopher Newport University, Newport News, VA, USA\fi}
\newcommand\Columbia[1] {\ifnum#1=1 12\else Department of Physics, Columbia University, New York, NY, USA\fi}
\newcommand\CUA[1] {\ifnum#1=1 13\else\fi}
\newcommand\CzechTechUniv[1] {\ifnum#1=1 14\else Czech Technical University in Prague, Faculty of Nuclear Sciences and Physical Engineering, Czech Republic\fi}
\newcommand\Duquesne[1] {\ifnum#1=1 15\else Duquesne University, Pittsburgh, PA, USA\fi}
\newcommand\Duke[1] {\ifnum#1=1 16\else\fi}
\newcommand\FIU[1] {\ifnum#1=1 17\else Florida International University, Miami, FL, USA\fi}
\newcommand\GeorgiaState[1] {\ifnum#1=1 18\else Georgia State University, Atlanta, GA, USA\fi}
\newcommand\Glasgow[1] {\ifnum#1=1 19\else School of Physics and Astronomy, University of Glasgow, Glasgow, UK\fi}
\newcommand\GSI[1] {\ifnum#1=1 20\else GSI Helmholtzzentrum fuer Schwerionenforschung, Darmstadt, Germany\fi}
\newcommand\GWU[1] {\ifnum#1=1 21\else The George Washington University, Washington, DC, USA\fi}
\newcommand\Hampton[1] {\ifnum#1=1 22\else\fi}
\newcommand\HEAROKEK[1] {\ifnum#1=1 23\else\fi}
\newcommand\HUJI[1] {\ifnum#1=1 24\else Racah Institute of Physics, Hebrew University, Jerusalem, Israel\fi}
\newcommand\IJCLabOrsay[1] {\ifnum#1=1 25\else Université Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\fi}
\newcommand\IMP[1] {\ifnum#1=1 26\else Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu, China\fi}
\newcommand\Inha[1] {\ifnum#1=1 27\else\fi}
\newcommand\IowaState[1] {\ifnum#1=1 28\else Iowa State University\fi}
\newcommand\IPAS[1] {\ifnum#1=1 29\else\fi}
\newcommand\JAEA[1] {\ifnum#1=1 30\else\fi}
\newcommand\JazanUniversity[1] {\ifnum#1=1 31\else Jazan University, Gizan, Jazan.\fi}
\newcommand\JeonbukNational[1] {\ifnum#1=1 32\else\fi}
\newcommand\JLab[1] {\ifnum#1=1 33\else\fi}
\newcommand\JMU[1] {\ifnum#1=1 34\else\fi}
\newcommand\KobeUniversity[1] {\ifnum#1=1 35\else Graduate School of Science, Kobe University, Kobe, Japan\fi}
\newcommand\KoreaUniversity[1] {\ifnum#1=1 36\else\fi}
\newcommand\Kyungpook[1] {\ifnum#1=1 37\else\fi}
\newcommand\LANL[1] {\ifnum#1=1 38\else Los Alamos National Laboratory, Los Alamos, NM, USA\fi}
\newcommand\LBNL[1] {\ifnum#1=1 39\else\fi}
\newcommand\LehighUniversity[1] {\ifnum#1=1 40\else Lehigh University, Bethlehem, PA, USA\fi}
\newcommand\LLNL[1] {\ifnum#1=1 41\else Lawrence Livermore National Laboratory, Livermore, CA, USA\fi}
\newcommand\MoreheadState[1] {\ifnum#1=1 42\else Morehead State University, Morehad, KY, USA\fi}
\newcommand\MIT[1] {\ifnum#1=1 43\else Massachusetts Institute of Technology, Cambridge, MA, USA\fi}
\newcommand\MSU[1] {\ifnum#1=1 44\else Mississippi State University, Mississippi State, MS, USA\fi}
\newcommand\NCKU[1] {\ifnum#1=1 45\else National Cheng Kung University, Tainan, Taiwan\fi}
\newcommand\NCU[1] {\ifnum#1=1 46\else National Central University, Chungli, Taiwan\fi}
\newcommand\Nihon[1] {\ifnum#1=1 47\else Nihon University, CST, Tokyo, Japan\fi}
\newcommand\NMSU[1] {\ifnum#1=1 48\else New Mexico State University, Las Cruces, NM, USA\fi}
\newcommand\NRNUMEPhI[1] {\ifnum#1=1 49\else National Research Nuclear University MEPhI, Moscow, Russian Federation\fi}
\newcommand\NRCN[1] {\ifnum#1=1 50\else Nuclear Research Center - Negev, Physics Dept., Beer-Sheva, Israel\fi}
\newcommand\NTHU[1] {\ifnum#1=1 51\else National Tsing Hua University, Hsinchu, Taiwan\fi}
\newcommand\NTU[1] {\ifnum#1=1 52\else National Taiwan University, Taipei, Taiwan\fi}
\newcommand\ODU[1] {\ifnum#1=1 53\else Old Dominion University, Department of Physics, Norfolk VA, USA\fi}
\newcommand\Ohio[1] {\ifnum#1=1 53\else Ohio University, Dept. Of Physics and Astronomy, Athens OH, USA\fi}
\newcommand\ORNL[1] {\ifnum#1=1 55\else Oak Ridge National Laboratory, PO Box 2008, Oak Ridge, TN, USA\fi}
\newcommand\PNNL[1] {\ifnum#1=1 56\else Pacific Northwest National Laboratory, Richland, WA, USA\fi}
\newcommand\Pusan[1] {\ifnum#1=1 57\else Pusan National Univeristy, Busan, Republic of Korea\fi}
\newcommand\Rice[1] {\ifnum#1=1 58\else Rice University, Houston, TX, USA\fi}
\newcommand\RIKEN[1] {\ifnum#1=1 59\else RIKEN Nishina Center, Wako, Saitama, Japan\fi}
\newcommand\Rutgers[1] {\ifnum#1=1 60\else The State University of New Jersey, Department of Physics and Astronomy, Piscataway, NJ, USA\fi}
\newcommand\Saha[1] {\ifnum#1=1 61\else\fi}
\newcommand\CFNS[1] {\ifnum#1=1 62\else Center for Frontiers in Nuclear Science, Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA\fi}
\newcommand\StonyBrook[1] {\ifnum#1=1 63\else Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA\fi}
\newcommand\RBRC[1] {\ifnum#1=1 64\else RIKEN BNL Research Center, Brookhaven National Laboratory, Upton, NY, USA\fi}
\newcommand\SCNU[1] {\ifnum#1=1 65\else\fi}
\newcommand\Seoul[1] {\ifnum#1=1 66\else Seoul National University, Seoul, Republic of Korea\fi}
\newcommand\Sejong[1] {\ifnum#1=1 67\else Sejong University, Seoul, Republic of Korea\fi}
\newcommand\Shinshu[1] {\ifnum#1=1 68\else Shinshu University, Matsumoto, Nagano, Japan\fi}
\newcommand\Sungkyunkwan[1] {\ifnum#1=1 69\else Sungkyunkwan University, Suwon, Republic of Korea\fi}
\newcommand\TAU[1] {\ifnum#1=1 70\else\fi}
\newcommand\Tokyo[1] {\ifnum#1=1 71\else\fi}
\newcommand\Tsinghua[1] {\ifnum#1=1 72\else Tsinghua University, Beijing, China\fi}
\newcommand\Tsukuba[1] {\ifnum#1=1 73\else Tsukuba University of Technology, Tsukuba, Ibaraki, Japan.\fi}
\newcommand\CUBoulder[1] {\ifnum#1=1 74\else University of Colorado Boulder, Boulder, CO, USA\fi}
\newcommand\UCAD[1] {\ifnum#1=1 75\else\fi}
\newcommand\UConn[1] {\ifnum#1=1 76\else University of Connecticut, Storrs, CT, USA\fi}
\newcommand\UH[1] {\ifnum#1=1 77\else University of Houston, Houston, TX, USA\fi}
\newcommand\UIUC[1] {\ifnum#1=1 78\else University of Illinois, Urbana, IL, USA\fi}
\newcommand\UKansas[1] {\ifnum#1=1 79\else\fi}
\newcommand\UKY[1] {\ifnum#1=1 80\else\fi}
\newcommand\Ljubljana[1] {\ifnum#1=1 81\else Faculty of Mathematics and Physics, University of Ljubljana, Ljubljana, Slovenia\fi}
\newcommand\NorthernGeorgia[1] {\ifnum#1=1 82\else\fi}
\newcommand\NewHampshire[1] {\ifnum#1=1 83\else University of New Hampshire, Durham, NH, USA\fi}
\newcommand\Oslo[1] {\ifnum#1=1 84\else Department of Physics, University of Oslo, Norway\fi}
\newcommand\Regina[1] {\ifnum#1=1 85\else University of Regina, Regina, SK, Canada\fi}
\newcommand\USeoul[1] {\ifnum#1=1 86\else University of Seoul, Seoul, Republic of Korea\fi}
\newcommand\USTC[1] {\ifnum#1=1 87\else\fi}
\newcommand\UTAustin[1] {\ifnum#1=1 88\fi}
\newcommand\UTsukuba[1] {\ifnum#1=1 89\else University of Tsukuba, Tsukuba, Japan\fi}
\newcommand\UTK[1] {\ifnum#1=1 90\else University of Tennessee, Knoxville, TN, USA\fi}
\newcommand\UTSM[1] {\ifnum#1=1 91\else\fi}
\newcommand\UVA[1] {\ifnum#1=1 92\else University of Virginia, Charlottesville, VA, USA\fi}
\newcommand\Vanderbilt[1] {\ifnum#1=1 93\else Department of Physics and Astronomy, Vanderbilt University, Nashville, TN, USA\fi}
\newcommand\VirginiaTech[1] {\ifnum#1=1 94\else\fi}
\newcommand\VirginiaUnion[1] {\ifnum#1=1 95\else Virginia Union University, Richmond, VA, USA\fi}
\newcommand\WayneState[1] {\ifnum#1=1 96\else Wayne State University, Detroit, MI, USA\fi}
\newcommand\WI[1] {\ifnum#1=1 97\else Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot, Israel\fi}
\newcommand\WandM[1] {\ifnum#1=1 98\else William and Mary, Williamsburg, VA, USA\fi}
\newcommand\Yamagata[1] {\ifnum#1=1 99\else Faculty of Science, Yamagata University, Yamagata, Japan\fi}
\newcommand\Yarmouk[1] {\ifnum#1=1 100\else\fi}
\newcommand\Yonsei[1] {\ifnum#1=1 101\else Yonsei University, Seoul, Republic of Korea\fi}
\newcommand\York[1] {\ifnum#1=1 102\else University of York, York, UK\fi}
\newcommand\Zagreb[1] {\ifnum#1=1 103\else Department of Physics, Faculty of Science, University of Zagreb, Zagreb, Croatia\fi}
